On the Complexity of Electromagnetic Far-Field Modeling

Modern wireless systems are envisioned to employ antenna architectures that not only transmit and receive electromagnetic (EM) waves, but also intentionally reflect and possibly transform incident EM waves. In this paper, we propose a mathematically rigorous framework grounded in Maxwell's equations for analyzing the complexity of EM far-field modeling of general antenna architectures. We show that-under physically meaningful assumptions-such antenna architectures exhibit limited complexity, i.e., can be modeled by finite-rank operators using finitely many parameters. Furthermore, we construct a sequence of finite-rank operators whose approximation error decays super-exponentially once the operator rank exceeds an effective bandwidth associated with the antenna architecture and the analysis frequency. These results constitute a fundamental prerequisite for the efficient and accurate modeling of general antenna architectures on digital computing platforms.

==> sty/eth-colors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% ETH Zürich's Corporate Design Colors
%%
%% Torben Kölle (tkoelle@iis.ee.ethz.ch)
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Corporate design colors extracted from the official website:
% https://ethz.ch/staffnet/en/service/communication/corporate-design/colours.html

% ETH blue:
\definecolor{eth_blue}{RGB}{33, 92, 175}
\definecolor{eth_blue_10}{RGB}{233, 239, 247}
\definecolor{eth_blue_20}{RGB}{211, 222, 239}
\definecolor{eth_blue_40}{RGB}{166, 190, 223}
\definecolor{eth_blue_60}{RGB}{122, 157, 207}
\definecolor{eth_blue_80}{RGB}{77, 125, 191}
\definecolor{eth_blue_120}{RGB}{8, 64, 126}

% ETH petrol:
\definecolor{eth_petrol}{RGB}{0, 120, 148}
\definecolor{eth_petrol_10}{RGB}{231, 244, 247}
\definecolor{eth_petrol_20}{RGB}{204, 228, 234}
\definecolor{eth_petrol_40}{RGB}{153, 202, 213}
\definecolor{eth_petrol_60}{RGB}{102, 175, 192}
\definecolor{eth_petrol_80}{RGB}{51, 149, 171}
\definecolor{eth_petrol_120}{RGB}{0, 89, 109}

% ETH green:
\definecolor{eth_green}{RGB}{98, 115, 19}
\definecolor{eth_green_10}{RGB}{239, 241, 231}
\definecolor{eth_green_20}{RGB}{224, 227, 208}
\definecolor{eth_green_40}{RGB}{192, 199, 161}
\definecolor{eth_green_60}{RGB}{161, 171, 113}
\definecolor{eth_green_80}{RGB}{129, 143, 66}
\definecolor{eth_green_120}{RGB}{54, 82, 19}

% ETH bronze:
\definecolor{eth_bronze}{RGB}{142, 103, 19}
\definecolor{eth_bronze_10}{RGB}{244, 240, 231}
\definecolor{eth_bronze_20}{RGB}{232, 225, 208}
\definecolor{eth_bronze_40}{RGB}{210, 194, 161}
\definecolor{eth_bronze_60}{RGB}{187, 164, 113}
\definecolor{eth_bronze_80}{RGB}{165, 133, 66}
\definecolor{eth_bronze_120}{RGB}{112, 79, 18}

% ETH red:
\definecolor{eth_red}{RGB}{183, 53, 45}
\definecolor{eth_red_10}{RGB}{248, 235, 234}
\definecolor{eth_red_20}{RGB}{241, 215, 213}
\definecolor{eth_red_40}{RGB}{226, 174, 171}
\definecolor{eth_red_60}{RGB}{212, 134, 129}
\definecolor{eth_red_80}{RGB}{197, 93, 87}
\definecolor{eth_red_120}{RGB}{150, 39, 45}

% ETH purple:
\definecolor{eth_purple}{RGB}{167, 17, 122}
\definecolor{eth_purple_10}{RGB}{248, 232, 243}
\definecolor{eth_purple_20}{RGB}{239, 208, 227}
\definecolor{eth_purple_40}{RGB}{220, 158, 201}
\definecolor{eth_purple_60}{RGB}{202, 108, 174}
\definecolor{eth_purple_80}{RGB}{183, 59, 146}
\definecolor{eth_purple_120}{RGB}{140, 10, 89}

% ETH grey:
\definecolor{eth_grey}{RGB}{111, 111, 111}
\definecolor{eth_grey_10}{RGB}{241, 241,241}
\definecolor{eth_grey_20}{RGB}{226, 226, 226}
\definecolor{eth_grey_40}{RGB}{197, 197, 197}
\definecolor{eth_grey_60}{RGB}{169, 169, 169}
\definecolor{eth_grey_80}{RGB}{140, 140, 140}
\definecolor{eth_grey_120}{RGB}{87, 87, 87}


==> sty/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Macros for the Paper 
%%
%% "A Sampling Theorem for EM Far-Field Models"
%%
%% Torben Kölle, Alexander Stutz, and Christoph Studer
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Color Palette:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sty/eth-colors}

% Corporate design colors:
% ETH blue:
\colorlet{blue}{eth_blue}
\colorlet{blue_10}{eth_blue_10}
\colorlet{blue_20}{eth_blue_20}
\colorlet{blue_40}{eth_blue_40}
\colorlet{blue_60}{eth_blue_60}
\colorlet{blue_80}{eth_blue_80}
\colorlet{blue_120}{eth_blue_120}
% ETH petrol:
\colorlet{petrol}{eth_petrol}
\colorlet{petrol_10}{eth_petrol_10}
\colorlet{petrol_20}{eth_petrol_20}
\colorlet{petrol_40}{eth_petrol_40}
\colorlet{petrol_60}{eth_petrol_60}
\colorlet{petrol_80}{eth_petrol_80}
\colorlet{petrol_120}{eth_petrol_120}
% ETH green:
\colorlet{green}{eth_green}
\colorlet{green_10}{eth_green_10}
\colorlet{green_20}{eth_green_20}
\colorlet{green_40}{eth_green_40}
\colorlet{green_60}{eth_green_60}
\colorlet{green_80}{eth_green_80}
\colorlet{green_120}{eth_green_120}
% ETH bronze:
\colorlet{bronze}{eth_bronze}
\colorlet{bronze_10}{eth_bronze_10}
\colorlet{bronze_20}{eth_bronze_20}
\colorlet{bronze_40}{eth_bronze_40}
\colorlet{bronze_60}{eth_bronze_60}
\colorlet{bronze_80}{eth_bronze_80}
\colorlet{bronze_120}{eth_bronze_120}
% ETH red:
\colorlet{red}{eth_red}
\colorlet{red_10}{eth_red_10}
\colorlet{red_20}{eth_red_20}
\colorlet{red_40}{eth_red_40}
\colorlet{red_60}{eth_red_60}
\colorlet{red_80}{eth_red_80}
\colorlet{red_120}{eth_red_120}
% ETH purple:
\colorlet{purple}{eth_purple}
\colorlet{purple_10}{eth_purple_10}
\colorlet{purple_20}{eth_purple_20}
\colorlet{purple_40}{eth_purple_40}
\colorlet{purple_60}{eth_purple_60}
\colorlet{purple_80}{eth_purple_80}
\colorlet{purple_120}{eth_purple_120}
% ETH grey:
\colorlet{grey}{eth_grey}
\colorlet{grey_10}{eth_grey_10}
\colorlet{grey_20}{eth_grey_20}
\colorlet{grey_40}{eth_grey_40}
\colorlet{grey_60}{eth_grey_60}
\colorlet{grey_80}{eth_grey_80}
\colorlet{grey_120}{eth_grey_120}

% Custom colors:
\definecolor{pink}{RGB}{214,82,130}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tikz Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclarepatternformonly{south east lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{5pt}{5pt}}{\pgfqpoint{5pt}{5pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{5pt}}
    \pgfpathlineto{\pgfqpoint{5pt}{0pt}}
    \pgfpathmoveto{\pgfqpoint{.2pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{-.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{5.2pt}{4.8pt}}
    \pgfpathlineto{\pgfqpoint{4.8pt}{5.2pt}}
    \pgfusepath{stroke}}
    
\pgfdeclarepatternformonly{horizontal lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3.54pt}{3.54pt}}{\pgfqpoint{3.54pt}{3.54pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{2pt}}
    \pgfpathlineto{\pgfqpoint{3.54pt}{2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal behind text}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{15pt}{15pt}}{\pgfqpoint{15pt}{15pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{15pt}{15pt}}
    \pgfpathmoveto{\pgfqpoint{14.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{15.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{14.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{15.2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal pattern node}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{3pt}{3pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{3pt}{3pt}}
    \pgfpathmoveto{\pgfqpoint{2.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{3.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{2.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{3.2pt}}
    \pgfusepath{stroke}}

\def\centerOfC at (#1,#2){
    \draw [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.27,-.27) rectangle (.27,.27);
    \draw [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.3,-.15) rectangle (.3,.15);
    \draw [shift={(#1,#2)},line width=0.3pt, fill=white] (0,0) ellipse (0.16 and 0.16);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (-0.2,0) -- (0.2,0);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (0,-0.2) -- (0,0.2);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (0:0.16) arc (0:90:.16) -- cycle;
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (180:0.16) arc (180:90+180:.16) -- cycle;
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Operators:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\diag}{diag}			            % diag matrix
\DeclareMathOperator{\Ex}{\mathbb{E}}		            % expectation operator
\DeclareMathOperator{\spn}{span}		                % span
\DeclareMathOperator{\range}{range}		                % range
\newcommand{\T}[0]{\mathsf{T}}                          % transpose
\newcommand{\He}[0]{\mathsf{H}}                         % hermitian
\DeclareMathOperator*{\argmin}{arg\,min}                % argmax
\DeclareMathOperator*{\maximize}{maximize}              % maximize               

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Font Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\up}[1]{{\textnormal{#1}}}                  % subscripts
\newcommand{\upc}[1]{{\textnormal{\textbf{#1}}}}        % subscripts in caption

\newcommand{\mat}[1]{{\bm{\mathbf{#1}}}}                % matrices
\newcommand{\vect}[1]{{\bm{\mathbf{#1}}}}               % vectors
\newcommand{\uvect}[1]{{\hat{\bm{\mathbf{#1}}}}}        % unit vectors
\newcommand{\oper}[1]{\mathbb{#1}}                      % operator

\newcommand{\phs}[1]{{\color{pink}\mathsf{#1}}}         % phasor scalar
\newcommand{\phv}[1]{{\color{pink}\bm{\mathsf{#1}}}}    % phasor vector

\newcommand{\set}[2]{\left\{#1\bigm\vert#2\right\}}     % set

% Temporary:
\newcommand{\norm}[2][]{\left\lVert#2\right\rVert_{#1}} %norm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Fancy Ref Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\fancyrefapplabelprefix}{app}		        % Appendix
\newcommand*{\fancyrefthmlabelprefix}{thm}		        % Theorem
\newcommand*{\fancyrefdefilabelprefix}{defi}            % Definition
\newcommand*{\fancyrefproplabelprefix}{prop}	        % Proposition
\newcommand*{\fancyrefalglabelprefix}{alg}		        % Algorithm
\newcommand*{\fancyrefasmlabelprefix}{asm}		        % Assumption
\newcommand*{\fancyrefremlabelprefix}{rem}		        % Remark

% Temporary:
\newcommand*{\fancyreflemlabelprefix}{lem}		% Lemma
\newcommand*{\fancyrefcorlabelprefix}{cor}		% Corollary

% Label names
\frefformat{vario}{\fancyrefseclabelprefix}{Section~#1}
\frefformat{vario}{\fancyrefthmlabelprefix}{Theorem~#1}
\frefformat{vario}{\fancyrefdefilabelprefix}{Definition~#1}
\frefformat{vario}{\fancyreffiglabelprefix}{Figure~#1}
\frefformat{vario}{\fancyrefapplabelprefix}{Appendix~#1}
\frefformat{vario}{\fancyrefeqlabelprefix}{(#1)}
\frefformat{vario}{\fancyrefproplabelprefix}{Proposition~#1}
\frefformat{vario}{\fancyrefalglabelprefix}{Algorithm~#1}
\frefformat{vario}{\fancyrefasmlabelprefix}{Assumption~#1}
\frefformat{vario}{\fancyrefremlabelprefix}{Remark~#1}

% Temporary:
\frefformat{vario}{\fancyreflemlabelprefix}{Lemma~#1}
\frefformat{vario}{\fancyrefcorlabelprefix}{Corollary~#1}

==> sty/tikz_style.tex <==
\tikzset{physical/.style={line width=0.3mm}}

\tikzset{
  current/.style={
    line width=0.3mm,
    postaction={decorate},
    decoration={
      markings,
      mark=at position 0.7 with {
        \arrow{Triangle[length=2.5mm,width=1.5mm]}
      }
    }
  }
}

\tikzset{hatched/.style={line width=0.25mm}}

\tikzset{
    field_arrow/.style={
    line width=0.3mm,
    color=white,
    postaction={decorate},
    decoration={
      markings,
      mark=at position 1 with {
        \arrow[draw=black,fill=red]{Triangle[length=2mm,width=1.5mm]}
      }
    }
  }
}

\tikzset{field/.style={line width=0.3mm}}

\tikzset{label_line/.style={line width=0.2mm}}
